Solving Robust MDPs through No-Regret Dynamics

Reinforcement Learning is a powerful framework for training agents to navigate different situations, but it is susceptible to changes in environmental dynamics. However, solving Markov Decision Processes that are robust to changes is difficult due to nonconvexity and size of action or state spaces. While most works have analyzed this problem by taking different assumptions on the problem, a general and efficient theoretical analysis is still missing. However, we generate a simple framework for improving robustness by solving a minimax iterative optimization problem where a policy player and an environmental dynamics player are playing against each other. Leveraging recent results in online nonconvex learning and techniques from improving policy gradient methods, we yield an algorithm that maximizes the robustness of the Value Function on the order of $\mathcal{O}\left(\frac{1}{T^{\frac{1}{2}}}\right)$ where $T$ is the number of iterations of the algorithm.

==> old/etash_robust_mdp.tex <==
\def\usebigfont{1}
\input{new_main}

==> old/etash_robust_mdp_large.tex <==
\def\usebigfont{1}
\input{new_main}

==> old/introduction.tex <==
\section{Introduction}
Reinforcement Learning (RL) is a powerful subset of machine learning that enables agents to learn through trial-and-error interactions with their environment. RL has succeeded in various applications such as game playing, robotics, and finance \citep{Sutton1998}. However, one of the main challenges of RL is its susceptibility to environmental changes. When a trained policy operates in different environmental dynamics than it was trained under, it often underperforms and achieves suboptimal rewards \citep{Farebrother2018, Packer2018, Cobbe2018,  Song2019, Raileanu2021}. 

To mitigate this problem, Robust MDPs have emerged as a promising solution to address the issue of the sensitivity of reinforcement learning to changing environments. By optimizing policies to have large value functions even in the worst-case environmental dynamics, Robust MDPs provide a more stable approach to training agents. There are different variants of robust MDPs, including distributionally robust MDPs \citep{xu2010distributionally, ruszczynski2010risk}, soft-robust MDPs \citep{buchholz2019light, Lobo2011}, and adversarial robustness \citep{pattanaik2017robust, eysenbach2021maximum}. Overall, robust MDPs have the potential to enhance the reliability of reinforcement learning in practical applications greatly.
% There are different variants of robust MDPs, including distributionally robust MDPs \citep{xu2010distributionally, ruszczynski2010risk, shapiro2016rectangular, xu2009parametric, petrik2012approximate, ghavamzadeh2016safe, chen2019distributionally}, soft-robust MDPs \citep{buchholz2019light, Lobo2011, steimle2021multi}, and adversarial robustness \citep{pattanaik2017robust, eysenbach2021maximum}.


Improving RL's robustness is crucial in ensuring AI safety. Mitigating disastrous failures of RL-trained agents in practice can prevent many undesirable outcomes \citep{Srinivasan2020, choi2021robust}. In several high-stakes environments, provable guarantees of robustness are paramount to preventing such undesirable outcomes. While the need for robust policies in RL is clear, finding them is challenging. The value function is highly nonconvex and is difficult to optimize with respect to policy and transition dynamics. Furthermore, the task is even more daunting when dealing with large state and action spaces, as finding algorithms that scale becomes an enormous challenge. 

Many existing solutions have made significant progress in finding efficient and accurate methodologies for solving Robust MDPs. Some of the first algorithms to solve Robust MDPs with guarantees and empirical performance are via transition dynamics set assumptions\citep{Nilim2003, iyengar2005robust}, Robust Policy Iteration \citep{Mankowitz2019, tamar2014scaling, sinha2016policy} or Robust Q-Learning \citep{wang2021online}; however, relatively few algorithms exist to solve this problem via policy gradient methods. Traditionally, policy gradient methods are popular due to their simplicity, stability, and scalability to large action and state spaces \citep{silver2014deterministic}. Furthermore, some policy gradient methods have achieved promising convergence results for solving Robust MDPs. However, due to the difficulty of nonconvex optimization, these frameworks still have suboptimal convergence and robustness guarantees. Moreover, many existing algorithms rely on strong assumptions on the uncertainty set of transitions, namely assuming rectangularity. Proving convergence bounds for more general uncertainty sets are notably difficult however.

However, a common framework for solving similar optimization problems with strong convergence guarantees is that of the Repeated Game Structure or No-Regret Dynamics. This models an optimization problem as a repeated game where one player tries to improve some objective function, and one tries to reduce the objective function \citep{hannan1957approximation, freund1996game, foster1999regret}. The advantage of such a framework is that its convergence is remarkably simple;  the two players converge to a correlated equilibrium in time proportional to the sum of their regrets \citep{ zinkevich2003online}. In fact, \citet{wang2022accelerated} showed that the margin or robustness of a linear classifier could be sufficiently improved over time using similar no-regret dynamics. We want to use a similar No-Reget Dynamics framework to generate Robust MDP algorithms. However, these frameworks often assume the games are convex-concave or even strongly-convex-strongly-concave. However, a Robust MDP is a notably nonconvex problem. 

 Recently, \citet{Suggala2019} showed that Follow the Perturbed Leader can achieve relatively strong regret even in the nonconvex case, provided that some minimization oracle is available. Incorporating this approach into a no-regret online framework, such as the one from no-regret dynamics, could lead to strong robustness. However, the minimization oracle is challenging to parameterize in general. Under gradient dominance assumptions of the value function, it is still possible to construct a minimization oracle, which allows for provable guarantees that the projected gradient ascent will converge to an optimal solution. Therefore, we model the optimization process for Robust MDPs as a game between policy and environmental dynamics players. Both utilize variants of Follow the Perturbed Leader and Projected Gradient Ascent.  

 In summary, we develop a novel nonconvex game framework with which we express the convergence of solving Robust MDPs under many different conditions and algorithms. We demonstrate that simply using FTPL with our framework achieves strongest convergence bounds for Robust MDPs with only a convex uncertainty set assumption while also enjoying the scalability of policy gradient techniques. We extend our framework to also demonstrate the convergence under settings where the value function is smooth or strongly-gradient dominated. To our knowledge, this is the first work to utilize strong gradient dominance to achieve stronger convergence for Robust MDPs. With the simplicity of our novel framework, we achieve the strongest convergence bounds with the fewest assumptions in the literature while also enjoying scalability.

\paragraph{Contributions}
Combining these, we have derived an efficient algorithm for solving Robust MDPs with provable guarantees of convergence that improve over existing algorithms. 
\begin{enumerate}
    \item We develop the a novel nonconvex No-Regret Dynamics framework suitable for solving nonconvex games.  We prove that the convergence of these nonconvex games to a robust minima in expectation is upper bounded by the sum of the regrets of the two players. This tool provided a general tool that we use to demonstrate convergence properties for many different algorithmic setups under many different conditions.
    \item We utilize this novel nonconvex game framework to design a solution process to Robust MDPs by modeling it as a two-player online game between a policy player and an environmental dynamics player, where the two players' regrets bound the robustness of the policies. Given the convergence is upper bounded by the regret, we demonstrate convergence when different optimization strategies are used by different players.
    \item When the policy player utilizes Follow the Perturbed Leader and the environmental dynamics player follows Best Response alongside an optimization oracle, we show the robustness is maximized at a rate of $\mathcal{O}\left(\frac{1}{T^{\frac{1}{2}}}\right)$. In the direct parameterization setting, we show that the loss functions seen by both players are Gradient Dominated, meaning we can use Projected Gradient Ascent as the optimization oracle. This achieves the optimal convergence in terms of $T$ while only needing a convex uncertainty set, relinquishing the common rectangularity assumption often seen in the literature with very simple convergence analysis. This also enjoys the benefit of scalability of policy gradient algorithms.
    \item When the difference between Robust MDPs objective function under different policies or environments is smooth, we improve Projected Gradient Ascent's convergence, improving both players' regrets. This setup includes changing the environment player to use Follow the Perturbed Leader Plus, a variant algorithm we generate. We also prove the regret bound of FTPL+. This also included proving that if the policy player employs the Optimistic Follow the Perturbed Leader algorithm,  its choices are stable and do not vary largely between timesteps. 
    \item We show that in cases where the Robust MDP satisfies "Strong Gradient Dominance," we can show that projected gradient ascent significantly improves its convergence rate, improving the convergence rate of the entire optimization algorithm. We demonstrate that a toy example of Regularized Robust MDPs satisfies this definition of "Strong Gradient Dominance." To our knowledge, this is the first work to study Strong Gradient Dominance in Robust MDPs. However, given the flexibility of our framework, the analysis is simple.
    
\end{enumerate}


==> onlinelearning.tex <==
\section{No Regret Dynamics}
We will now formally introduce the main theoretical tool that drives our analysis: No Regret Dynamics. Given our algorithm can be viewed as 

==> sampling.tex <==
\section{Intelligent Sampling}
Notably, our goal for sampling the rewards for each state is to reduce the difference between our estimate $\hPt(s_k)$ and $\trueV(s_k)$. If this error is $0$ for example, we know our gradients and losses are deterministic, significantly improving the convergence rate of our algorithm. However, there is often error in practice. In this section, we will quantify this error and then introduce a sampling pattern as a way to compute $H_t$ such that estimation error is minimized.

\subsection{Error in Value Function Estimate}
The process of solving the Value Function for all states in a finite-horizon MDP with a finite amount of states is equivalent to solving a system of linear equations. For the true Value Function value $\trueV$, we have that for any state $s$
$$V_W^{\pi}(s) - \gamma \sum_{a \in \A}\pi(a, s) \sum_{s' \in \Sc} \Pw(s', a, s)V_W^{\pi}(s')= R(s) \text{.}$$

Similarly, we have $\mM \hat{\mathbf{v}} = \hat{\mR}$ where $\hat{\mathbf{v}}$ is the vectorized form of $\hPt$. Therefore, if we want to bound the error, we can decompose this estimate into the noise and signal terms. Namely, 
\begin{align}
    \mM \hat{\mathbf{v}} &= \hat{\mR}\\
    \mM (\mathbf{v} + \mathbf{e}) &= \mR + \mathbf{n}\\
    \mM \mathbf{e} &= \mathbf{n}\\
    \mathbf{e} &= \mM^{-1}\mathbf{n}
\end{align}
Here, $\sigma$ is the error in the $\hat{\mR}$ and $\mathbf{e}$ is the error in the $\hat{\mathbf{v}}$. Therefore, let's say we want to minimize the error term of the value function for the initial state, $\me_0 = \mM_0^{-1}\mathbf{n}$. Here, we introduce a simple assumption about the noise 
\begin{assumption}
    \label{ass:noisevar} We assume that any given sample of the reward function for any state is a probability distribution with expected value at the true reward $R(s_k)$ with variance $\sigma^2$.
\end{assumption}
Therefore, any given element $n_i$ is a random variable with expected value $0$ and variance $\frac{\sigma^2}{H_t(s_i)}$. 

\begin{align}
    \me_0 &= \mM_0^{-1}\mathbf{n} \\
    &= \sum_i \mM_{0, i}^{-1}\mathbf{n}_i\\
    &\leq \sum_i |\mM_{0, i}^{-1}| |\mathbf{n}_i|\\
    &\leq  \sum_i |\mM_{0, i}^{-1}| \frac{\psi\sigma^2}{H_t(s_i)} \label{eq:minimization}
\end{align}

where the last inequality comes from applying Chebyshev's inequality and, thus, holds with probability at least $1 - \frac{1}{\psi^2}$. Finding the optimal $H_t$ that minimizes \Cref{eq:minimization} such that the sum of $H_t$ is bounded above by some constant $\lambda$ yields
\begin{restatable}{lemma}{minsam}
    \label{lem:minsam}
    The minimizing solution to \begin{align}
        \underset{H_t}{\argmin} & \sum_i |\mM_{0, i}^{-1}| \frac{\psi\sigma^2}{H_t(s_i)}\\
        &\text{ s.t. } \sum_k H_t(s_k) \leq \lambda \\
        &\text{ s.t. } H_t(s_k) \geq 0\; \forall k
    \end{align}
    is $$H_t(s_i) = \frac{\sqrt{|\mM_{0, i}^{-1}|}}{\lambda \sum_k^K \sqrt{|\mM_{0, k}^{-1}|}}\text{.}$$ This solution achieves the minimum of 
    $$\sum_i |\mM_{0, i}^{-1}| \frac{\psi\sigma^2}{H_t(s_i)} = \frac{\left(\sum_i \sqrt{\psi\sigma^2|\mM_{0, k}^{-1}|}\right)^2}{\lambda}$$
\end{restatable} 

\Cref{lem:minsam} states that we need only sample a total of $\lambda$ states in order to get an error bound. 



  nnn
